Training One Model to Master Cross-Level Agentic Actions via Reinforcement Learning

The paradigm of agentic AI is shifting from engineered complex workflows to post-training native models. However, existing agents are typically confined to static, predefined action spaces-such as exclusively using APIs, GUI events, or robotic commands. This rigidity limits their adaptability in dynamic environments where the optimal granularity of interaction varies contextually. To bridge this gap, we propose CrossHA, a unified agentic model that masters heterogeneous action spaces and autonomously selects the most effective interface for each step of a trajectory. We introduce a comprehensive training pipeline that integrates cold-start supervised fine-tuning with a Multi-Turn Group Relative Policy Optimization (GRPO) algorithm. This approach enables the agent to learn adaptive action switching-balancing high-level efficiency with low-level precision-without human-specified rules. Extensive experiments on over 800 tasks in the open-world Minecraft environment demonstrate that CrossHA achieves state-of-the-art performance. By dynamically leveraging the strengths of diverse action spaces, our model significantly outperforms fixed-action baselines, exhibiting superior generalization and efficiency in long-horizon reasoning. All code and models are available at https://github.com/CraftJarvis/OpenHA.

==> defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}



==> tables/not_used/deepha_main.tex <==
\begin{table*}[]
    \centering
    \caption{
    % Evaluation results of Minecraft agents. 
    % For every group, we report the success rate of a representative task, the finished ratio of all available tasks (\textit{FT}) and the average success rates across all tasks (\textit{ASR}). 
    Evaluation results of Minecraft agents on over 800 tasks.
    For each task category, we report the success rate on a representative task (indicated by the icon), the percentage of Finished Tasks within the category (\textit{FT}), and the Average Success Rate across all tasks in that category (\textit{ASR} $\pm$ standard deviation). Results highlighted in {\color{blue}{blue}} represent the second-best performances, while those in {\color{red}{red}} indicate the state-of-the-art performance for each metric across all agents. `-' signifies tasks where the agent failed to achieve any success.
    }
    \label{tab:main_results}
    \resizebox{\textwidth}{!}{%
    \renewcommand\arraystretch{1.4}
    \begin{tabular}{@{}lccccccccccccccc@{}}
    \toprule
     & \multicolumn{3}{c}{Mine Blocks} &  & \multicolumn{3}{c}{Kill Entities} &  & \multicolumn{3}{c}{Craft Items} &  & \multicolumn{3}{c}{Smelt Items} \\ \cmidrule(l){2-4} \cmidrule(l){6-8} \cmidrule(l){10-12} \cmidrule(l){14-16}  
    \multirow{-2}{*}{Method} & \includegraphics[scale=0.04,valign=c]{minecraft/oak_log.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.16,valign=c]{minecraft/spider.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.08,valign=c]{minecraft/wooden_pickaxe.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.04,valign=c]{minecraft/iron_ingot.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ \\ \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{E1EAFF}{\textbf{\textit{Instruction-Conditioned Policies}}}} \\
    VPT~\citep{vpt} & 20.0 & 30.7 & $6.0^{\pm11.4}$ &  & 10.0 & 24.6 & $3.6^{\pm7.7}$ &  & N/A & 6.7 & $0.8^{\pm3.3}$ &  & 0.0 & 0.0 & $0.0^{\pm0.0}$ \\
    STEVE-I~\citep{steve1} & 50.0 & 29.4 & $8.0^{\pm17.0}$ &  & 0.0 & 14.7 & $3.9^{\pm12.0}$ &  & 0.0 & 16.4 & $3.2^{\pm8.4}$ &  & 0.0 & 0.0 & $0.0^{\pm0.0}$ \\
    ROCKET-1~\citep{rocket1} & 60.0 & 57.5 & $18.9^{\pm24.3}$ &  & 60.0 & 63.9 & $27.9^{\pm29.3}$ &  & - & - & - &  & - & - & - \\
    JARVIS-VLA~\citep{jarvisvla} & 55.0 & 55.3 & $30.0^{\pm35.4}$ &  & 60.0 & 61.9 & $18.5^{\pm22.7}$ &  & 40.0 & \textcolor{blue}{\textbf{74.3}} & $25.1^{\pm23.9}$ &  & 60.0 & \textcolor{blue}{\textbf{92.3}} & $65.4^{\pm32.3}$ \\ 
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{F0FBEF}{\textbf{\textit{Hierarchical Agents}}}} \\
    LanguageHA~\citep{palme} & 60.0 & 31.3 & $11.3^{\pm14.5}$ 
    &  & 0.0 & 12.8 & $6.5^{\pm9.3}$ 
    &  & 5.0 & 19.3 & $6.3^{\pm9.2}$ 
    &  & 0.0 & 0.0 & $0.0^{\pm0.0}$ \\

    PointHA~\citep{rocket1} & \textcolor{blue}{\textbf{90.0}} & 61.0 & \textcolor{blue}{\textbf{$37.1^{\pm38.5}$}} 
        &  & 50.0 & \textcolor{blue}{\textbf{90.1}} & $26.5^{\pm23.4}$ 
        &  & 15.0 & 27.5 & $6.7^{\pm10.8}$ 
        &  & 10.0 & 37.0 & $5.0^{\pm8.7}$ \\
    
    MotionHA~\citep{rth} & 70.0 & 51.0 & $27.4^{\pm35.2}$ 
        &  & 20.0 & 29.5 & $4.3^{\pm10.8}$ 
        &  & 0.0 & 0.0 & $0.0^{\pm0.0}$ 
        &  & 0.0 & 0.0 & $0.0^{\pm0.0}$ \\
    
    LatentHA~\citep{omnijarvis} & 70.0 & 54.2 & $24.4^{\pm31.1}$ 
        &  & 50.0 & 24.6 & $8.5^{\pm17.9}$ 
        &  & 0.0 & 19.1 & $3.0^{\pm7.5}$ 
        &  & 0.0 & 2.2 & $0.2^{\pm1.5}$ \\
    OpenHA~\citep{wang2025openha} & 80.0 & \textcolor{blue}{{\textbf{67.3}}} & $30.1^{\pm13.9}$ 
        &  & \textcolor{blue}{\textbf{70.0}} & 62.6 & \textcolor{blue}{\textbf{$32.5^{\pm9.2}$}} 
        &  & \textcolor{blue}{\textbf{80.0}} & 58.8 & \textcolor{blue}{\textbf{$31.9^{\pm13.7}$}} 
        &  & \textcolor{blue}{\textbf{75.0}} & \textcolor{blue}{\textbf{92.3}} & \textcolor{blue}{\textbf{$66.6^{\pm28.1}$}} \\
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{FEF1F1}{\textbf{\textit{Ours}}}} \\
    DeepHA & \textcolor{red}{\textbf{100.0}} & \textcolor{red}{\textbf{82.4}} & \textcolor{red}{\textbf{$48.9^{\pm43.6}$}} 
    &  & \textcolor{red}{\textbf{90.0}} & \textcolor{red}{\textbf{92.3}} & \textcolor{red}{\textbf{$38.9^{\pm45.3}$}} 
    &  & \textcolor{red}{\textbf{75.0}} & \textcolor{red}{\textbf{85.6}} & \textcolor{red}{\textbf{$43.2^{\pm26.5}$}} 
    &  & \textcolor{red}{\textbf{90.0}} & \textcolor{red}{\textbf{93.5}} & \textcolor{red}{\textbf{$82.4^{\pm22.6}$}} \\
    \bottomrule
    \end{tabular}%
    }
% \vspace{-0.2 in}
\end{table*}


    % DHA (w/o CoA) & $75.$ & \color{blue}{{$75.8$}} & \color{blue}{{$42.4^{\pm35.9}$}}  &   &  \color{blue}{{$70.$}}  &  \color{blue}{{$90.2$}}  &  \color{blue}{{$28.7^{\pm25.3}$}} &   &  \color{blue}{{$65.$}} &  \color{red}{\textbf{$75.6$}}  & \color{red}{\textbf{$28.6^{\pm29.5}$}}  &   &  \color{blue}{\textbf{$80.$}}  &  \color{red}{\textbf{$93.5$}} & \color{blue}{\textbf{$72.3^{\pm45.3}$}} \\ % choose the best one of one group of belowing models
    % DHA (Raw) & $75.$ &  $61.0$ & $35.5^{\pm26.5}$ &  & $70.$ & $63.9$ &  $21.5^{\pm13.3}$  &   &  $65.$ & $75.6$ & $28.6^{\pm29.5}$  &   & $80.$ & $93.5$ & $72.3^{\pm45.3}$ \\
    % DHA (Motion) & $75.$ & $75.8$ & $42.4^{\pm35.9}$  &   & $45.$ & $50.8$ &  $9.1^{\pm15.8}$ &   &  $0.$ & $0.0$ & $0.0^{\pm0.0}$  &   & $0.$  &  $0.0$ & $0.0^{\pm0.0}$ \\
    % DHA (Grounding) & $100.$ & $78.4$ & $39.6^{\pm35.6}$ &   & $70.$ & $90.2$ & $28.7^{\pm25.3}$ &  & $25.$ & $35.5$ & $12.5^{\pm13.3}$ &  & $20.$  &  $57.0$ & $23.0^{\pm25.3}$ \\

==> tables/not_used/generalization_ablation_COPY.tex <==

\begin{table*}[]
    \centering
    \caption{
        The evaluation results of RL agents across Out-of-distribution tasks. The metrics and notation follow \autoref{tab:main_results}.
    }
    \label{tab:generalization_ablations}
    \resizebox{\textwidth}{!}{%
    \renewcommand\arraystretch{1.4}
    \begin{tabular}{@{}lcccccccccccccc@{}}
    \begin{tabular}{@{}lcccccccccccccc@{}}
    \toprule
     & \multicolumn{3}{c}{Mine Blocks} &  & \multicolumn{3}{c}{Kill Entities} &  & \multicolumn{3}{c}{Craft Items} & & \multicolumn{2}{c}{All Tasks}\\ \cmidrule(l){2-4} \cmidrule(l){6-8} \cmidrule(l){10-12} \cmidrule(l){14-15}
    \multirow{-2}{*}{Method} & \includegraphics[scale=0.04,valign=c]{minecraft/oak_log.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.16,valign=c]{minecraft/spider.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.08,valign=c]{minecraft/wooden_pickaxe.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  &\textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ \\ \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{FFF9D9}{\textbf{\textit{RL  Agents}}}} \\
    RawHA-RL & 81.8 & 29.2 & $28.9^{\pm44.2}$ 
    &  & 50.0 & 55.1 & $28.4^{\pm32.3}$ 
    &  & \textbf{\color{red}{100.0}} & 71.3 & $69.8^{\pm44.4}$ & & 51.9 &\textbf{\color{blue}{$42.4^{\pm{45.1}}$}}\\
    GroundingHA-RL & 88.9 & 29.4 & $27.2^{\pm42.4}$
        &  & \textbf{\color{red}{72.7}} & 51.0 & \textbf{\color{red}{$33.9^{\pm35.9}$}}
        &  & 83.3 & 58.5 & $57.2^{\pm48.1}$ & & 41.0 &$39.4^{\pm{44.3}}$\\
    MotionHA-RL & \textbf{\color{red}{100.0}} & 47.4 & \textbf{\color{red}{$41.5^{\pm45.5}$}}
        &  & 66.7 & 61.2 & $26.8^{\pm26.7}$ 
        &  & 74.2 & 52.9 & $49.0^{\pm47.3}$ & & 43.8 &$39.1^{\pm{42.0}}$\\
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{FEF1F1}{\textbf{\textit{Ours}}}} \\
    CrossAgent(w/o STRL stage) 
    & 63.6 & 35.1 & \textbf{\color{blue}{$39.0^{\pm46.5}$}} 
    & & 30.5& 33.3 & $22.2^{\pm42.6}$ 
    & & 57.1 & 55.7 & \textbf{\color{blue}{$58.0^{\pm48.4}$}} & & 41.4 &\textbf{\color{blue}{$39.7^{\pm{48.1}}$}}\\
    CrossAgent & \textbf{\color{red}{94.7}} & 45.2 & \textbf{\color{red}{$40.0^{\pm48.3}$}}
    & & \textbf{\color{blue}{61.6}} & 57.1 & \textbf{\color{blue}{$28.4^{\pm33.2}$}} 
    & & \textbf{\color{red}{83.3}} & \textbf{\color{blue}{72.7}} & \textbf{\color{red}{$78.8^{\pm41.0}$}} & & 58.3 &\textbf{\color{red}{$49.1^{\pm46.6}$}}\\
    \bottomrule
    \end{tabular}%
}
% \vspace{-0.2 in}
\end{table*}



\begin{table*}[]
    \centering
    \caption{
        The evaluation results of RL agents across in-distribution tasks. The metrics and notation follow \autoref{tab:main_results}.
    }
    \label{tab:generalization_ablations}
    \resizebox{\textwidth}{!}{%
    \renewcommand\arraystretch{1.4}
    \begin{tabular}{@{}lcccccccccccccc@{}}
    \toprule
     & \multicolumn{3}{c}{Mine Blocks} &  & \multicolumn{3}{c}{Kill Entities} &  & \multicolumn{3}{c}{Craft Items} & & \multicolumn{2}{c}{All Tasks}\\ \cmidrule(l){2-4} \cmidrule(l){6-8} \cmidrule(l){10-12} \cmidrule(l){14-15}
    \multirow{-2}{*}{Method} & \includegraphics[scale=0.08,valign=c]{cvpr2026/minecraft/crafting_table.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.16,valign=c]{cvpr2026/minecraft/sheep.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.04,valign=c]{cvpr2026/minecraft/enchanting_table.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  &\textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ \\ \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{FFF9D9}{\textbf{\textit{RL  Agents}}}} \\
    RawHA-RL & 45.7 & 90.0 & $65.2^{\pm32.1}$ 
    &  & 85.7  & 80.0 & $41.6^{\pm21.8}$
    &  & 93.0 & 100.0 & $96.2^{\pm3.8}$ & & 90.0 &$70.1^{\pm{33.6}}$\\
    GroundingHA-RL & 31.4 & 90.0 & $46.8^{\pm35.6}$
        &  & 77.8 & 90.0 & $48.8^{\pm34.5}$
        &  & 74.7 & 100.0 & $69.3^{\pm28.4}$ & & 93.3 &$52.6^{\pm{31.5}}$\\
    MotionHA-RL & 42.6 & 100.0 & $78.6^{\pm24.6}$
        &  & 81.6 & 90.0 & $44.0^{\pm25.2}$ 
        &  & 38.8 & 100.0 & $63.0^{\pm20.7}$ & & 96.7 &$61.9^{\pm{27.5}}$\\
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{FEF1F1}{\textbf{\textit{Ours}}}} \\ d
    CrossAgent(w/o STRL stage) 
    & 56.2 & 100.0 & $63.3^{\pm28.9}$ 
    & & 62.7& 60.0 & $24.0^{\pm26.4}$ 
    & & 91.7 & 100.0 & $76.1^{\pm27.2}$ & & 86.6 &$39.7^{\pm{48.1}}$\\
    CrossAgent & 36.5 &90.0 & $70.7^{\pm33.3}$
    & & 85.6 & 90.0 & $52.1^{\pm22.9}$ 
    & & 90.0 & 100 & $83.7^{\pm25.5}$ & & 93.3 &$68.8^{\pm30.5}$\\
    \bottomrule
    \end{tabular}%
}
% \vspace{-0.2 in}
\end{table*}


==> tables/not_used/ogn_in_domain_table.tex <==
\begin{table*}[]
    \centering
    \caption{
        The evaluation results of RL agents across online tasks. The metrics and notation follow \ref{tab:main_results}.
    }
    \label{tab:in_domain_table}
    \resizebox{\textwidth}{!}{%
    \renewcommand\arraystretch{1.4}
    \begin{tabular}{@{}lcccccccccccccc@{}}
    \toprule
     & \multicolumn{3}{c}{Mine Blocks} &  & \multicolumn{3}{c}{Kill Entities} &  & \multicolumn{3}{c}{Craft Items} & & \multicolumn{2}{c}{All Tasks}\\ \cmidrule(l){2-4} \cmidrule(l){6-8} \cmidrule(l){10-12} \cmidrule(l){14-15}
    \multirow{-2}{*}{Method} & \includegraphics[scale=0.04,valign=c]{minecraft/oak_log.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.16,valign=c]{minecraft/spider.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.08,valign=c]{minecraft/wooden_pickaxe.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  &\textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ \\ \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{E1EAFF}{\textbf{\textit{Instruction-Conditioned Policies}}}}\\
    VPT~\citep{vpt} & 20.0 & 30.7 & $6.0^{\pm11.4}$ &  & 10.0 & 24.6 & $3.6^{\pm7.7}$ &  & 0.0 & 6.7 & $0.8^{\pm3.3}$& & 20.7 &$3.5^{\pm8.4}$\\
    STEVE-I~\citep{steve1} & 50.0 & 29.4 & $8.0^{\pm17.0}$ &  & 0.0 & 14.7 & $3.9^{\pm12.0}$ &  & 0.0 & 16.4 & $3.2^{\pm8.4}$& & 20.2 & $5.0^{\pm12.4}$\\
    ROCKET-1~\citep{rocket1} & 60.0 & 57.5 & $18.9^{\pm24.3}$ &  & 60.0 & \textbf{\color{blue}{63.9}} & $27.9^{\pm29.3}$ &  & 0.0 & 0.0 & $0.0^{\pm{0.0}}$& & 45.5 &$15.6^{\pm{24.9}}$\\
    JARVIS-VLA~\citep{jarvisvla} & 55.0 & 55.3 & $30.0^{\pm35.4}$ &  & 60.0 & 61.9 & $18.5^{\pm22.7}$ &  & 40.0 & \textbf{\color{red}{74.3}} & $25.1^{\pm23.9}$& & \textbf{\color{red}{63.8}} &$24.5^{\pm{28.4}}$\\ 
    %DeepHA & 100.0 & 82.4 & $48.9^{\pm43.6}$ 
    %&  & 90.0 & 92.3 & $38.9^{\pm45.3}$ 
    %&  & 75.0 & 85.6 & \textcolor{red}{\textbf{$43.2^{\pm26.5}$}}\\
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{F0FBEF}{\textbf{\textit{Hierarchical Agents}}}}\\
    RawHA~\citep{palme} & 60.0 & 36.3 & $27.2^{\pm38.2}$ 
    &  & 0.0 & 19.2 & $8.7^{\pm23.7}$ 
    &  & 50.0 & 43.9 & $26.0^{\pm35.2}$ & & 33.1 &$20.6^{\pm{34.0}}$\\
    GroundingHA~\citep{rocket1} & 90.0 & \textbf{\color{blue}{61.0}} & $37.1^{\pm38.5}$
        &  & 50.0 & \textbf{\color{red}{90.1}} & $26.5^{\pm23.4}$ 
        &  & 15.0 & 27.5 & $6.7^{\pm10.8}$ & & 59.5 &$23.4^{\pm{29.6}}$\\
    MotionHA~\citep{rth} & 70.0 & 51.0 & $27.4^{\pm35.2}$ 
        &  & 20.0 & 29.5 & $4.3^{\pm10.8}$ 
        &  & 0.0 & 0.0 & $0.0^{\pm0.0}$ & & 29.8 &$10.6^{\pm{24.4}}$\\
    LanguageHA~\citep{palme} & 60.0 & 31.3 & $11.3^{\pm14.5}$ 
    &  & 0.0 & 12.8 & $6.5^{\pm9.3}$ 
    &  & 5.0 & 19.3 & $6.3^{\pm9.2}$ & & 21.1 &$8.0^{\pm{11.5}}$\\
    LatentHA~\citep{omnijarvis} & 70.0 & 54.2 & $24.4^{\pm31.1}$ 
        &  & 50.0 & 24.6 & $8.5^{\pm17.9}$ 
        &  & 0.0 & 19.1 & $3.0^{\pm7.5}$ & & 32.6 &$12.0^{\pm{23.0}}$\\
    OpenHA~\citep{wang2025openha} & 80.0 & \textbf{\color{red}{67.3}} & $30.1^{\pm13.9}$ 
        &  & \textbf{\color{blue}{70.0}} & 62.6 & \textbf{\color{blue}{$32.5^{\pm9.2}$}}
        &  & 80.0 & 58.8 & $31.9^{\pm13.7}$ & & \textbf{\color{blue}{62.8}} &$31.5^{\pm{12.5}}$\\
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{FFF9D9}{\textbf{\textit{RL  Agents}}}} \\
    RawHA-RL & 81.8 & 29.2 & $28.9^{\pm44.2}$ 
    &  & 50.0 & 55.1 & $28.4^{\pm32.3}$ 
    &  & \textbf{\color{red}{100.0}} & 71.3 & $69.8^{\pm44.4}$ & & 51.9 &\textbf{\color{blue}{$42.4^{\pm{45.1}}$}}\\
    GroundingHA-RL & 88.9 & 29.4 & $27.2^{\pm42.4}$
        &  & \textbf{\color{red}{72.7}} & 51.0 & \textbf{\color{red}{$33.9^{\pm35.9}$}}
        &  & 83.3 & 58.5 & $57.2^{\pm48.1}$ & & 41.0 &$39.4^{\pm{44.3}}$\\
    MotionHA-RL & \textbf{\color{red}{100.0}} & 47.4 & \textbf{\color{red}{$41.5^{\pm45.5}$}}
        &  & 66.7 & 61.2 & $26.8^{\pm26.7}$ 
        &  & 74.2 & 52.9 & $49.0^{\pm47.3}$ & & 43.8 &$39.1^{\pm{42.0}}$\\
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{FEF1F1}{\textbf{\textit{Ours}}}} \\
    CrossAgent(w/o STRL stage) 
    & 63.6 & 35.1 & $39.0^{\pm46.5}$ 
    & & 30.5& 33.3 & $22.2^{\pm42.6}$ 
    & & 57.1 & 55.7 & $58.0^{\pm48.4}$ & & 41.4 &$39.7^{\pm{48.1}}$\\
    CrossAgent & \textbf{\color{blue}{94.7}} & 45.2 & \textbf{\color{blue}{$40.0^{\pm48.3}$}}
    & & 56.2 & 57.1 & $28.4^{\pm33.2}$ 
    & & \textbf{\color{blue}{83.3}} & \textbf{\color{blue}{72.7}} & \textbf{\color{red}{$78.8^{\pm41.0}$}} & & 58.3 &\textbf{\color{red}{$49.1^{\pm46.6}$}}\\
    \bottomrule
    \end{tabular}%
}
% \vspace{-0.2 in}
\end{table*}


==> tables/not_used/ogn_main_result.tex <==
\begin{table*}[]
    \centering
    \caption{
        The evaluation results of Minecraft agents across more than 800 tasks are presented.For each task category, we report three metrics: the success rate of a representative task (indicated by its icon), the percentage of tasks that the agent succeeds at least once (FT), and the average success rate across all tasks in the category (ASR) with standard deviation. Results highlighted in {\color{blue}{blue}} correspond to the second-best performances, while those in {\color{red}{red}} represent the state-of-the-art performance for each metric across all agents. A `-' symbol denotes tasks where the agent failed to achieve any success.
    }
    \label{tab:mai_results}
    \resizebox{\textwidth}{!}{%
    \renewcommand\arraystretch{1.4}
    \begin{tabular}{@{}lccccccccccc@{}}
    \toprule
     & \multicolumn{3}{c}{Mine Blocks} &  & \multicolumn{3}{c}{Kill Entities} &  & \multicolumn{3}{c}{Craft Items}\\ \cmidrule(l){2-4} \cmidrule(l){6-8} \cmidrule(l){10-12}
    \multirow{-2}{*}{Method} & \includegraphics[scale=0.04,valign=c]{minecraft/oak_log.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.16,valign=c]{minecraft/spider.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$ &  & \includegraphics[scale=0.08,valign=c]{minecraft/wooden_pickaxe.png} & \textit{FT} $\uparrow$ & \textit{ASR} $\uparrow$\\ \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{E1EAFF}{\textbf{\textit{Instruction-Conditioned Policies}}}}\\
    VPT~\citep{vpt} & 20.0 & 30.7 & $6.0^{\pm11.4}$ &  & 10.0 & 24.6 & $3.6^{\pm7.7}$ &  & - & 6.7 & $0.8^{\pm3.3}$\\
    STEVE-I~\citep{steve1} & 50.0 & 29.4 & $8.0^{\pm17.0}$ &  & 0.0 & 14.7 & $3.9^{\pm12.0}$ &  & 0.0 & 16.4 & $3.2^{\pm8.4}$\\
    ROCKET-1~\citep{rocket1} & 60.0 & 57.5 & $18.9^{\pm24.3}$ &  & 60.0 & \textbf{\color{blue}{63.9}} & $27.9^{\pm29.3}$ &  & - & - & -\\
    JARVIS-VLA~\citep{jarvisvla} & 55.0 & 55.3 & $30.0^{\pm35.4}$ &  & 60.0 & 61.9 & $18.5^{\pm22.7}$ &  & 40.0 & \textbf{\color{red}{74.3}} & $25.1^{\pm23.9}$\\ 
    %DeepHA & 100.0 & 82.4 & $48.9^{\pm43.6}$ 
    %&  & 90.0 & 92.3 & $38.9^{\pm45.3}$ 
    %&  & 75.0 & 85.6 & \textcolor{red}{\textbf{$43.2^{\pm26.5}$}}\\
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{F0FBEF}{\textbf{\textit{Hierarchical Agents}}}} \\
    RawHA~\citep{palme} & 60.0 & 36.3 & $27.2^{\pm38.2}$ 
    &  & 0.0 & 19.2 & $8.7^{\pm23.7}$ 
    &  & 50.0 & 43.9 & $26.0^{\pm35.2}$ \\
    GroundingHA~\citep{rocket1} & 90.0 & \textbf{\color{blue}{61.0}} & $37.1^{\pm38.5}$
        &  & 50.0 & \textbf{\color{red}{90.1}} & $26.5^{\pm23.4}$ 
        &  & 15.0 & 27.5 & $6.7^{\pm10.8}$ \\
    MotionHA~\citep{rth} & 70.0 & 51.0 & $27.4^{\pm35.2}$ 
        &  & 20.0 & 29.5 & $4.3^{\pm10.8}$ 
        &  & 0.0 & 0.0 & $0.0^{\pm0.0}$ \\
    LanguageHA~\citep{palme} & 60.0 & 31.3 & $11.3^{\pm14.5}$ 
    &  & 0.0 & 12.8 & $6.5^{\pm9.3}$ 
    &  & 5.0 & 19.3 & $6.3^{\pm9.2}$ \\
    LatentHA~\citep{omnijarvis} & 70.0 & 54.2 & $24.4^{\pm31.1}$ 
        &  & 50.0 & 24.6 & $8.5^{\pm17.9}$ 
        &  & 0.0 & 19.1 & $3.0^{\pm7.5}$ \\
    OpenHA~\citep{wang2025openha} & 80.0 & \textbf{\color{red}{67.3}} & $30.1^{\pm13.9}$ 
        &  & \textbf{\color{blue}{70.0}} & 62.6 & \textbf{\color{blue}{$32.5^{\pm9.2}$}}
        &  & 80.0 & 58.8 & $31.9^{\pm13.7}$ \\
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{FFF9D9}{\textbf{\textit{RL  Agents}}}} \\
    RawHA-RL & 81.8 & 29.2 & $28.9^{\pm44.2}$ 
    &  & 50.0 & 55.1 & $28.4^{\pm32.3}$ 
    &  & \textbf{\color{red}{100.0}} & 71.3 & $69.8^{\pm44.4}$ \\
    GroundingHA-RL & 88.9 & 29.4 & $27.2^{\pm42.4}$
        &  & \textbf{\color{red}{72.7}} & 51.0 & \textbf{\color{red}{$33.9^{\pm35.9}$}}
        &  & 83.3 & 58.5 & $57.2^{\pm48.1}$ \\
    MotionHA-RL & \textbf{\color{red}{100.0}} & 47.4 & \textbf{\color{red}{$41.5^{\pm45.5}$}}
        &  & 66.7 & 61.2 & $26.8^{\pm26.7}$ 
        &  & 74.2 & 52.9 & $49.0^{\pm47.3}$ \\
    \midrule
    \multicolumn{16}{l}{\cellcolor[HTML]{FEF1F1}{\textbf{\textit{Ours}}}} \\
    CrossAgent(w/o STRL stage) 
    & 63.6 & 35.1 & $39.0^{\pm46.5}$ 
    & & 30.5& 33.3 & $22.2^{\pm42.6}$ 
    & & 57.1 & 55.7 & $58.0^{\pm48.4}$ \\
    CrossAgent & \textbf{\color{blue}{94.7}} & 45.2 & \textbf{\color{blue}{$40.0^{\pm48.3}$}}
    & & 56.2 & 57.1 & $28.4^{\pm33.2}$ 
    & & \textbf{\color{blue}{83.3}} & \textbf{\color{blue}{72.7}} & \textbf{\color{red}{$78.8^{\pm41.0}$}} \\
    \bottomrule
    \end{tabular}%
}
% \vspace{-0.2 in}
\end{table*}


